Denoising Task Difficulty-based Curriculum for Training Diffusion Models

Diffusion-based generative models have emerged as powerful tools in the realm of generative modeling. Despite extensive research on denoising across various timesteps and noise levels, a conflict persists regarding the relative difficulties of the denoising tasks. While various studies argue that lower timesteps present more challenging tasks, others contend that higher timesteps are more difficult. To address this conflict, our study undertakes a comprehensive examination of task difficulties, focusing on convergence behavior and changes in relative entropy between consecutive probability distributions across timesteps. Our observational study reveals that denoising at earlier timesteps poses challenges characterized by slower convergence and higher relative entropy, indicating increased task difficulty at these lower timesteps. Building on these observations, we introduce an easy-to-hard learning scheme, drawing from curriculum learning, to enhance the training process of diffusion models. By organizing timesteps or noise levels into clusters and training models with ascending orders of difficulty, we facilitate an order-aware training regime, progressing from easier to harder denoising tasks, thereby deviating from the conventional approach of training diffusion models simultaneously across all timesteps. Our approach leads to improved performance and faster convergence by leveraging benefits of curriculum learning, while maintaining orthogonality with existing improvements in diffusion training techniques. We validate these advantages through comprehensive experiments in image generation tasks, including unconditional, class-conditional, and text-to-image generation.

==> figures/convergence.tex <==

\begin{wrapfigure}[14]{r}{0.383\textwidth}
    \centering
    \vspace{-20mm}
    \includegraphics[width=\linewidth]{figures/figure_files/convergence.pdf}
    \vspace{-7mm}
    \caption{
    The models trained using the proposed curriculum learning approach demonstrate faster convergence compared to vanilla models, irrespective of evaluation metrics. 
    }
    \label{fig:convergence}
\end{wrapfigure}

==> tables/model_size.tex <==
\begin{wraptable}[12]{r}{0.48\textwidth}
    \centering
    % \vspace{-8mm}
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
    \multicolumn{5}{l}{\bf{Class-Conditional ImageNet} 256$\times$256.} \\
    \toprule
    Model & FID$\downarrow$  & IS$\uparrow$  & Prec$\uparrow$ & Rec$\uparrow$ \\
    \toprule
    DiT-S/2  & 43.30 & 33.63 & 0.42 & 0.54 \\
    DiT-S/2 + Ours  & \cellcolor{gray!15}\textbf{39.66} &  \cellcolor{gray!15}\textbf{36.57} & \cellcolor{gray!15}\textbf{0.44} & \cellcolor{gray!15}\textbf{0.54} \\
    \arrayrulecolor{gray}\cmidrule(lr){1-5}
    DiT-B/2 & 30.27 & 60.06 & 0.55 & 0.52 \\
    DiT-B/2 + Ours & \cellcolor{gray!15}\textbf{22.96} & \cellcolor{gray!15}\textbf{75.98} & \cellcolor{gray!15}\textbf{0.62} & \cellcolor{gray!15}\textbf{0.52} \\
    \arrayrulecolor{gray}\cmidrule(lr){1-5}
    DiT-L/2 & 11.18 & 146.95 & 0.75 & 0.47 \\
    DiT-L/2 + Ours & \cellcolor{gray!15}\textbf{8.18} & \cellcolor{gray!15}\textbf{186.37} & \cellcolor{gray!15}\textbf{0.79} & \cellcolor{gray!15}\textbf{0.47} \\
    \arrayrulecolor{black}\bottomrule
    \end{tabular}%
    }
    % \vspace{-2mm}
    \caption{Note that curriculum learning achieves consistent improvements across model sizes.
    }
    \label{tab:model_size}
\end{wraptable}


==> tables/xl_result.tex <==
\begin{wraptable}[8]{r}{0.43\textwidth}
    \centering
    % \vspace{-7mm}
    \resizebox{0.43\textwidth}{!}{%

    \begin{tabular}{llcccc}
    \toprule
    \multicolumn{5}{l}{\bf{Class-Conditional ImageNet} 256$\times$256.} \\
    \toprule
    \multicolumn{2}{l}{Model}  & FID$\downarrow$ & IS$\uparrow$ & Prec$\uparrow$ & Rec$\uparrow$  \\
    \midrule
    & DiT-XL/2  & 9.40 & 166.83 & 0.7709 & 0.4865 \\
    % \cmidrule(lr){1-6}
    & DiT-XL/2 + Ours &\cellcolor{gray!15}\textbf{}  &\cellcolor{gray!15}\textbf{}  &\cellcolor{gray!15}\textbf{}	  &\cellcolor{gray!15}\textbf{}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-1mm}
    \caption*{\textbf{Table A: }Comparative results on DiT-XL/2. 
    }
    \label{tab:xl_result}
\end{wraptable}


